Support in the domain of numerical algorithms in the education of future secondary school mathematics teachers

This article presents web-based applets designed primarily to educate future mathematics teachers in the field of numerical algorithms and, secondarily, to serve high school students themselves. The applets allow users to explore the behaviour of basic numerical algorithms as applied to fundamental mathematical topics taught at high schools. The advantage is that no software is required, and students can intuitively test how a given method works by adjusting specific problem parameters, not only by viewing a list of approximate solutions, but especially through graphical output. Furthermore, they have access to multiple different methods for comparison.

==> definitions.tex <==
% Document template for students' assignments
% Šablona dokumentu pro studentské samostatné práce
% -- common definitions 
% (c) 2006-2022, Jan Pospíšil <honik@kma.zcu.cz>

% uncomment only the definitions needed in your document

% --------------------------------------------- %
% ----- New Definitions and Abbreviations ----- %
% --------------------------------------------- %

% ----- New useful definitions:

% \newcommand{\field}[1]{\mathbf{#1}}
% \newcommand{\mtrx}[1]{\mathbb{#1}}
% %\newcommand{\mtrx}[1]{\mathrm{#1}}
% \newcommand{\attractor}[1]{\mathcal{#1}}
% % - operators
\DeclareMathOperator{\Cov}{Cov}
% \DeclareMathOperator{\Diff}{Diff}
% \DeclareMathOperator{\Dom}{Dom}
% \DeclareMathOperator{\Law}{Law}
% \DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Var}{Var}
% \DeclareMathOperator{\erf}{erf}
% \DeclareMathOperator{\fix}{fix}
% \DeclareMathOperator{\per}{per}
% \newcommand{\ddt}[1]{\dfrac{d {#1}}{dt}}
% \newcommand{\pd}[2]{\dfrac{\partial {#1}}{\partial {#2}}}
% % - vectors
% \newcommand{\aveckonj}[3]{{#1}\vec{{#2}_1}\wedge{#1}\vec{{#2}_2}\wedge\dots\wedge{#1}\vec{{#2}_{#3}}}
% \newcommand{\aveclist}[3]{{#1}\vec{{#2}_1},{#1}\vec{{#2}_2},\dots,{#1}\vec{{#2}_{#3}}}
% \newcommand{\nVec}[1]{[{#1}_1, {#1}_2, \dots, {#1}_n]^T}
% \newcommand{\veckonj}[2]{\vec{{#1}_1}\wedge\vec{{#1}_2}\wedge\dots\wedge\vec{{#1}_{#2}}}
% \newcommand{\veclist}[2]{\vec{{#1}_1},\vec{{#1}_2},\dots,\vec{{#1}_{#2}}}
% % - others
% \newcommand{\atxzero}[1]{\left.{#1}\right|_{\vec{x}=\vec{x_0}}}
% \newcommand{\composition}[1]{{#1}\circ{#1}\circ\dots\circ{#1}}
% \newcommand{\lkmax}[1]{\lambda_{\max}^{({#1})}}
% \newcommand{\scalar}[2]{\left\langle{#1},{#2}\right\rangle}

% ----- Used Abbreviations:

\newcommand{\ds}{\displaystyle}
\renewcommand{\d}{\,\mathrm{d}} % differential
\newcommand{\dx}{\,\mathrm{d}x}
\newcommand{\dt}{\,\mathrm{d}t}
\newcommand{\e}{\mathrm{e}}     % Euler number
\newcommand{\E}{\mathbb{E}}     % Expectation
\newcommand{\F}{\mathcal{F}}    % sigma algebra, filtration

\DeclareMathOperator{\logp}{log1p}
\newcommand{\NaN}{\mathrm{NaN}}

% - matrices 
%\newcommand{\A}{\mtrx{A}}
%\newcommand{\B}{\mtrx{B}}
%\newcommand{\E}{\mathbb{E}}	% Expected value
%\newcommand{\I}{\mtrx{I}}	% Identity
%\newcommand{\M}{\mtrx{M}}
%\renewcommand{\P}{\mtrx{P}}
%\newcommand{\V}{\mtrx{V}}
% - spaces
%\newcommand{\3}{\mathcal{E}}	% step functions
%\newcommand{\B}{\mathcal{B}}	% Borel sets
%\newcommand{\Cn}{\C^n}
%\newcommand{\Ctem}{\C_\text{tem}}
%\newcommand{\C}{\mathcal{C}}	% Continuous whatever
%\newcommand{\Diffr}{\Diff^r(\Rn)}
%\newcommand{\F}{\mathcal{F}}	% Filtration
%\newcommand{\G}{\mathcal{G}}
%\newcommand{\HuS}{\mathcal{S}}	% Hu's space
%\newcommand{\Normal}{\mathcal{N}} % Normal Gaussian Distribution
\newcommand{\N}{\mathbf{N}}	% Positive Integers
\renewcommand{\P}{\mathbb{P}}	% Probability (measure)
\newcommand{\R}{\mathbf{R}}	% Real numbers
%\newcommand{\Rm}{\R^m}
%\newcommand{\Rn}{\R^n}
%\newcommand{\Timeset}{\mathbf{T}}
%\newcommand{\U}{\mathcal{U}}	% Hilbert
%\newcommand{\V}{\mathcal{V}}	% Hilbert
%\newcommand{\Z}{\field{Z}}	% Integers
%\renewcommand{\L}{\mathcal{L}}	% Linear whatever
% - orbits
%\newcommand{\orbit}{O_{\vec{f}}\,(\vec{x_0})}
%\newcommand{\porbit}{O^+_{\vec{f}}(\vec{x_0})}
%\newcommand{\norbit}{O^-_{\vec{f}}(\vec{x_0})}
% - words abbrevs
%\newcommand{\dimensional}[1]{\ensuremath{#1}\nobreakdash-dimensional\ }
%\newcommand{\kdim}{\dimensional{k}}
%\newcommand{\ndim}{\dimensional{n}}
%\newcommand{\onedim}{\dimensional{1}}
%\newcommand{\infdim}{\dimensional{\infty}}
%\newcommand{\alim}{$\alpha$\nobreakdash-limit\ }
%\newcommand{\olim}{$\omega$\nobreakdash-limit\ }
%\newcommand{\Poin}{Poincar\'e\ }
% - others
%\renewcommand{\bar}{\tilde}
%\renewcommand{\bar}{\relax}
%\newcommand{\attA}{\attractor{A}}
%\newcommand{\rarr}{\rightarrow}
%\newcommand{\darr}{\downarrow}
%\newcommand{\eps}{\varepsilon}
%\newcommand{\Laplace}{\Delta}
%\newcommand{\asP}{\mbox{a.s.-$\Prob$}}

% ----- Theorem-like environments:

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{acknowledgement}[theorem]{Acknowledgement} 
%\newtheorem{algorithm}[theorem]{Algorithm} 
%\newtheorem{axiom}[theorem]{Axiom} 
%\newtheorem{case}[theorem]{Case} 
%\newtheorem{claim}[theorem]{Claim} 
%\newtheorem{conclusion}[theorem]{Conclusion} 
%\newtheorem{condition}[theorem]{Condition} 
%\newtheorem{conjecture}[theorem]{Conjecture} 
%\newtheorem{corollary}[theorem]{Corollary} 
%\newtheorem{criterion}[theorem]{Criterion} 
%\newtheorem{definition}[theorem]{Definition} 
%\newtheorem{example}[theorem]{Example} 
%\newtheorem{exercise}[theorem]{Exercise} 
%\newtheorem{hypothesis}[theorem]{Hypothesis} 
%\newtheorem{lemma}[theorem]{Lemma} 
%\newtheorem{notation}[theorem]{Notation} 
%\newtheorem{problem}[theorem]{Problem} 
%\newtheorem{proposition}[theorem]{Proposition} 
%\newtheorem{question}[theorem]{Question} 
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{solution}[theorem]{Solution} 
%\newtheorem{summary}[theorem]{Summary} 
%\newtheorem{Rem}[theorem]{Remark}

\addto\captionsczech{%
  \def\theoremname{V\v{e}ta}%
  \def\definitionname{Definice}%
  \def\examplename{P\v{r}\'{\i}klad}%
  \def\remarkname{Pozn\'{a}mka}%
  \def\propositionname{Tvrzen\'{\i}}%
  \def\lemmaname{Lemma}%
  \def\corollaryname{D\r{u}sledek}%
}%
\addto\captionsenglish{%
  \def\theoremname{Theorem}%
  \def\definitionname{Definition}%
  \def\examplename{Example}%
  \def\remarkname{Remark}%
  \def\propositionname{Proposition}%
  \def\lemmaname{Lemma}%
  \def\corollaryname{Corollary}%
}%

\theoremstyle{definition}
       \newtheorem{dfn}{\definitionname}[section]
       \newtheorem{eg}{\examplename}[section]
\theoremstyle{remark}
       \newtheorem{rmk}{\remarkname}[section]
\theoremstyle{plain}
       \newtheorem{thm}{\theoremname}[section]
       \newtheorem{prop}[thm]{\propositionname}
       \newtheorem{lem}[thm]{\lemmaname}
       \newtheorem{cor}[thm]{\corollaryname}

\newcommand{\nocontentsline}[3]{}%


==> preamble.tex <==

\makeatletter

% ------------------------------------------------- %
% -----             Used Packages             ----- %
% ------------------------------------------------- %

% --- Proper encoding and language
\usepackage[latin2]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[czech,english]{babel}

% --- Geometry (Page layout), Graphicx, Hyperref
\usepackage{geometry}
\usepackage{ifpdf}
\ifpdf
        \@ifpackageloaded{hyperref}{}{\usepackage[pdftex]{hyperref}}
	\@ifpackageloaded{xcolor}{}{\usepackage[pdftex,svgnames,table]{xcolor}}
        \@ifpackageloaded{graphicx}{}{\usepackage[pdftex]{graphicx}}
	\usepackage{epstopdf}
\else
        \@ifpackageloaded{hyperref}{}{\usepackage[hypertex]{hyperref}}
	\@ifpackageloaded{xcolor}{}{\usepackage[dvips,svgnames,table]{xcolor}}
        \@ifpackageloaded{graphicx}{}{\usepackage[dvips]{graphicx}}
\fi
\graphicspath{{fig/}}

%\hypersetup{colorlinks=false,hidelinks=true}
%\hypersetup{colorlinks=true,allcolors=myblue}
\hypersetup{
    breaklinks=true,
    colorlinks=true,
    linkcolor=myblue,
    citecolor=myblue,
    urlcolor=myblue,
    unicode,
    naturalnames
}

\usepackage{xurl} % allow long url line breaks
% \usepackage{subcaption}

% --- Fonts
\usepackage{amssymb,amsfonts}
\usepackage{lmodern}

\def\foliofont{\fontsize{8}{10}\selectfont}

% --- Headings
\usepackage{fancyhdr}

% --- AMS Math
\usepackage{amsmath,amsthm,amscd,upref}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs=true} % number only equations that are referenced in the text

\let\ubar=\underline

% --- Improved lists
\usepackage{paralist} % enumerate with style
%\usepackage{enumerate} 
%\usepackage{enumitem}

% --- Improved tabulars and tables
%\usepackage{array,tabularx,hhline,dcolumn}
%\usepackage{booktabs}
%\usepackage{multirow}

% --- Improved figures
%\usepackage{wrapfig}
%\usepackage{caption}
%\usepackage{subcaption}
\usepackage{tikz}

% --- Text positioning
%\usepackage[absolute,overlay,showboxes]{textpos}
%\usepackage[absolute,overlay]{textpos}
%\setlength{\TPHorizModule}{1mm}
%\setlength{\TPVertModule}{1mm}
%\setlength{\parindent}{0mm}

% --- Bibliography and index
%\usepackage{makeidx}
% For author-year citations use:
% \usepackage{natbib}
% \usepackage[round,sort]{natbib}
 \usepackage[authoryear,round,sort]{natbib}
 \bibliographystyle{plainnat}
% For numbered citations use:
%\usepackage[square,sort,numbers]{natbib}

%%%\bibpunct[, ]{(}{)}{;}{a}{}{,}
\let\oldcite=\cite
\let\oldcitep=\citep
\let\oldcitet=\citet
\renewcommand\cite[1]{\hypersetup{linkcolor=Navy}\hyperlink{#1}{\oldcite{#1}}}
\renewcommand{\citet}[1]{\@ifstar{\hypersetup{linkcolor=Navy}\hyperlink{#1}{\oldcitet*{#1}}}
{\hypersetup{linkcolor=Navy}\hyperlink{#1}{\oldcitet{#1}}}}
\renewcommand{\citep}[1]{\hypersetup{linkcolor=Navy}\hyperlink{#1}{\oldcitep*{#1}}}
\renewcommand{\citet}[1]{\hypersetup{linkcolor=Navy}\hyperlink{#1}{\oldcite*{#1}}}
\let\bibfont\relax
\def\bibfont{\fontsize{8}{10}\selectfont}
\setlength{\bibsep}{0pt}
\newcommand{\citeauthornohref}[1]{{\protect\NoHyper\citeauthor{#1}\protect\endNoHyper}}
\newcommand{\Citeauthornohref}[1]{{\protect\NoHyper\Citeauthor{#1}\protect\endNoHyper}}
\newcommand{\doi}[1]{DOI~\href{\detokenize{https://doi.org/#1}}{\detokenize{#1}}}
\newcommand{\zblnumber}[1]{Zbl~\href{\detokenize{https://zbmath.org/?q=an:#1}}{\detokenize{#1}}}
\newcommand{\mrnumber}[1]{\href{\detokenize{https://www.ams.org/mathscinet-getitem?mr=#1}}{\detokenize{MR#1}}}
\newcommand{\arXiv}[2]{arXiv:\href{\detokenize{https://arxiv.org/abs/#1}}{\detokenize{#1 [#2]}}}
\newcommand{\msc}[1]{\href{https://mathscinet.ams.org/mathscinet/msc/msc2020.html?s=#1}{#1}}
\newcommand{\acm}[1]{\href{https://www.acm.org/publications/computing-classification-system/1998/#1}{\uppercase{#1}}}
\newcommand{\jel}[1]{\href{https://www.aeaweb.org/jel/guide/jel.php}{#1}}% TODO: better URL, see javascript function 'track' inside the page, it uses POST

% --- Appendices
%\usepackage[toc,page]{appendix}

% --- MATLAB listings
\usepackage{listings}
\lstset{language=Matlab,%       
    basicstyle=\ttfamily,
    breaklines=true,%
    morekeywords={quadl,integral},
    keywordstyle={\bfseries\color{blue}},%
    morekeywords=[2]{1}, keywordstyle=[2]{\color{black}},
    identifierstyle=\color{black},%
    stringstyle=\color{mylilas},
    commentstyle=\color{mygreen},%
    showstringspaces=false,%without this there will be a symbol in the places where there is a space
    numbers=none,%
    numberstyle={\tiny \color{black}},% size of the numbers
    numbersep=9pt, % this defines how far the numbers are from the text
    %emph=[1]{for,end,break},emphstyle=[1]\color{red}, %some words to emphasise
    %emph=[2]{word1,word2}, emphstyle=[2]{style},
    frame=single,
}

% --- Colors
% \definecolor{myblue}{rgb}{0,0,0.5} % Navy
\colorlet{myblue}{Navy}
% \definecolor{myblue}{rgb}{0.1,0.1,0.5}% darker blue
\definecolor{favorange}{cmyk}{0.02,0.22,1.0,0.15}
\definecolor{lightyellow}{cmyk}{0,0,0.1,0}

\definecolor{myfullred}{RGB}{244,63,43}
\definecolor{myhalfred}{RGB}{158,22,7}
\definecolor{myfullorange}{RGB}{255,128,0}
\definecolor{myhalforange}{RGB}{147,73,0}
\definecolor{mygreen}{RGB}{70,180,5}
\definecolor{mylilas}{RGB}{170,55,241}

%\colorlet{pagebgcolor}{lightyellow}
\colorlet{pagebgcolor}{white}
\colorlet{textcolor}{black}
\colorlet{titlebgcolor}{pagebgcolor}

% --- Check the citations and references
%\usepackage{refcheck}
%\usepackage[notcite]{showkeys}
%\usepackage{varioref,refstyle}
\usepackage{xspace}

% --- Highlighting text
\usepackage{soul}
\sethlcolor{LimeGreen}
\def\NEW{\hl}
\DeclareRobustCommand{\TODO}[1]{{\sethlcolor{yellow}\hl{TODO: #1}}}
\DeclareRobustCommand{\COMPLETED}[1]{{\sethlcolor{lime}\hl{COMPLETED: #1}}}
\DeclareRobustCommand{\FIXME}[1]{{\sethlcolor{Tomato}\hl{FIXME: #1}}}
\DeclareRobustCommand{\hlc}[1]{{\sethlcolor{cyan}\hl{#1}}}
\DeclareRobustCommand{\hlm}[1]{\colorbox{yellow}{$\displaystyle #1$}}
% to be able to highlight a text that contains \cite, \ref, \pageref, \eqref
\soulregister\cite7%
\soulregister\citep7%
\soulregister\eqref7%
\soulregister\pageref7%
\soulregister\ref7%

% --- Metadata
% Optional PDF information
\newcommand{\jpPdfInfo}{%
\ifpdf
\hypersetup{
  pdftitle={\jpTitle},
  pdfauthor={\jpAuthors},
  pdfkeywords={\jpKeywords},
  pdfinfo={
      MSC={\jpMSC},
      ACM={\jpACM},
      JEL={\jpJEL}
  }
}
\fi
}

% Cross journals compatibility:
\def\received#1{Received~#1\par}
\def\revised#1{Revised~#1\par}
\def\accepted#1{Accepted~#1\par}
\def\published#1{Published~#1\par}
\@ifundefined{ccode}{%
\newcommand{\ccode}[2]{\par
        \vspace*{8pt}
        {{\leftskip18pt\rightskip\leftskip
        \noindent{\it #1}\/: #2\par}}\par}
}{}
% macros \keywords and \email already exist in amsart
\@ifundefined{keywords}{\newcommand{\keywords}[1]{\ccode{Keywords}{#1}}}{}
\@ifundefined{email}{\newcommand{\email}[1]{\href{mailto:#1}{#1}}}{}

% Implementing switch cases in LaTeX:
% https://tex.stackexchange.com/questions/64131/implementing-switch-cases
\usepackage{xifthen}
\newboolean{default}
\newcommand{\case}{}
\newcommand{\default}{}
\newenvironment{switch}[1]{%
    \setboolean{default}{true}
    \renewcommand{\case}[2]{\ifthenelse{\equal{#1}{##1}}{%
        \setboolean{default}{false}##2}{}}%
    \renewcommand{\default}[1]{\ifthenelse{\boolean{default}}{##1}{}}
}{}

% ------------------------------------------------- %
% ----- Define Page Layout and Fancy Headings ----- %
% ------------------------------------------------- %
\@ifclassloaded{article}{%

% ----- Define page layout
%\geometry{twoside}
\geometry{a4paper,top=20mm,left=20mm,right=20mm,bottom=20mm} %,headsep=5mm}
\setlength{\headheight}{18.0pt} % overleaf warning
%\usepackage{showframe}

% ----- Define headings and foots
\rhead[]{\fancyplain{}{\slshape\rightmark}}
\chead{}
\lhead[\fancyplain{}{\slshape\leftmark}]{}
\cfoot{\fancyplain{\bfseries --~\thepage~--}{\bfseries --~\thepage~--}}

% --- Author block (for titlepage)
\usepackage{authblk}
%\usepackage[auth-sc]{authblk}
\renewcommand\Affilfont{\normalfont\small}

% ----- Define some structure commands
\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {2.3ex \@plus.2ex}%
                                   {\color{myblue}\normalfont\Large\bfseries }}

}{}% if article

\@ifclassloaded{beamer}{%
% theme
\usetheme{default}
% \setbeamercovered{%
% invisible
% %transparent,
% %still covered={\opaqueness<>{100}}
% }
\setbeamertemplate{navigation symbols}{}
\setbeamertemplate{sidebar left}{\rlap{\hskip1mm\insertlogo}}
\setbeamertemplate{sidebar right}{}
% \setbeamertemplate{headline}{}
\newcommand{\myfootlinefull}
{%
  \leavevmode%
  \hbox{\begin{beamercolorbox}[wd=\paperwidth,ht=2.5ex,dp=1.125ex,leftskip=3mm,rightskip=3mm]{author in head/foot}%
  \usebeamerfont{author in head/foot}\insertshortdate\hfill\insertshortauthor:\:
  \usebeamerfont{title in head/foot}\insertshorttitle\hfill \insertframenumber~/~\inserttotalframenumber
  \end{beamercolorbox}}%
  \vskip0pt%
}
\newcommand{\myfootlinenotitle}
{%
  \leavevmode%
  \hbox{\begin{beamercolorbox}[wd=\paperwidth,ht=2.5ex,dp=1.125ex,leftskip=3mm,rightskip=3mm]{author in head/foot}%
  \usebeamerfont{author in head/foot}\insertshortdate%\hfill\insertshortauthor:\:
  %\usebeamerfont{title in head/foot}\insertshorttitle
  \hfill \insertframenumber~/~\inserttotalframenumber
  \end{beamercolorbox}}%
  \vskip0pt%
}
\setbeamertemplate{footline}{\myfootlinefull}
%\setbeamercolor{normal text}{bg=lightyellow}
\setbeamercolor{background canvas}{bg=pagebgcolor}
\setbeamercolor{alerted text}{fg=Navy}
\setbeamercolor{structure}{fg=Navy}
\setbeamercolor{frametitle}{fg=textcolor}
%\setbeamercolor{title}{fg=textcolor}
\setbeamercolor{author in head/foot}{fg=textcolor}
\setbeamertemplate{frametitle}[default][right,rightskip=1mm]
\addtobeamertemplate{frametitle}{}{\noindent\makebox[\linewidth]{\textcolor{favorange}{\rule{\paperwidth}{1pt}}}}
\setbeamerfont{title}{shape=\scshape}
% \setbeamercolor{structure}{fg=black}
% \setbeamercolor{bibliography entry author}{fg=Navy}
% \setbeamercolor{bibliography entry title}{fg=Navy} 
% \setbeamercolor{bibliography entry location}{fg=Navy} 
% \setbeamercolor{bibliography entry note}{fg=Navy}  

\setbeamertemplate{bibliography item}{}
\setbeamersize{text margin left=5mm,text margin right=5mm}

\addtobeamertemplate{theorem begin}{%
    \setbeamercolor{block title}{fg=black,bg=favorange}%
    \setbeamercolor{block body}{fg=black,bg=lightyellow}%
}{}

\logo{%
\begin{tabular}{p{26mm}p{30mm}}%
\vspace{0mm}\href{http://www.fav.zcu.cz/en}{\includegraphics[height=13mm,trim=5mm 5mm 7mm 5mm,clip]{logo-fav_en}}&%
\vspace{1.5mm}\href{http://www.kma.zcu.cz/en}{\includegraphics[height=13mm,trim=0mm 0mm 135mm 0mm,clip]{logo-kma_en}}
\end{tabular}
}
\titlegraphic{%
\begin{tabular}{p{26mm}p{30mm}p{70mm}}%
\vspace{0mm}\href{http://www.fav.zcu.cz/en}{\includegraphics[height=13mm,trim=5mm 5mm 7mm 5mm,clip]{logo-fav_en}}&%
\vspace{1.5mm}\href{http://www.kma.zcu.cz/en}{\includegraphics[height=13mm,trim=0mm 0mm 135mm 0mm,clip]{logo-kma_en}}&%
\vspace{0mm}\hfill\href{http://www.ntis.zcu.cz/en}{\includegraphics[height=13mm,trim=0mm 0mm 0mm 0mm,clip]{logo-ntis}}
\end{tabular}
}

}{} % if beamer

% ----- New numbering
%\renewcommand\thesection{\alph{section}.}
%\renewcommand\thesubsection{\Alph{section}.\arabic{subsection}}
%\renewcommand{\thechapter}{\@Roman\c@chapter}
%\renewcommand{\thesection}{\@arabic\c@section}
%\renewcommand{\labelenumi}{(\roman{enumi})}
%\renewcommand{\fnum@figure}{{\bfseries\figurename~\thefigure}}
%\renewcommand{\fnum@table}{{\bfseries\tablename~\thetable}}

% ----------------------------------------------- %
% ----- Define Index and Bibliography style ----- %
% ----------------------------------------------- %

% change bibliography style right before \bibliography, e.g.
%\bibliographystyle{plainnat}
%\bibliographystyle{jp+doi+mr+zbl}
%\bibliographystyle{jd}
\setlength{\bibsep}{0pt}
%\makeindex

% ----------------------------------------------- %
% ----- Common definitions and macros       ----- %
% ----------------------------------------------- %
%\IfFileExists{definitions.tex}{
\input{definitions}
%}{}

% ----- Do NOT Allow changes in commands with '@'
\makeatother


